EXPLORER: Exploration-guided Reasoning for Textual Reinforcement Learning

Text-based games (TBGs) have emerged as an important collection of NLP tasks, requiring reinforcement learning (RL) agents to combine natural language understanding with reasoning. A key challenge for agents attempting to solve such tasks is to generalize across multiple games and demonstrate good performance on both seen and unseen objects. Purely deep-RL-based approaches may perform well on seen objects; however, they fail to showcase the same performance on unseen objects. Commonsense-infused deep-RL agents may work better on unseen data; unfortunately, their policies are often not interpretable or easily transferable. To tackle these issues, in this paper, we present EXPLORER which is an exploration-guided reasoning agent for textual reinforcement learning. EXPLORER is neurosymbolic in nature, as it relies on a neural module for exploration and a symbolic module for exploitation. It can also learn generalized symbolic policies and perform well over unseen data. Our experiments show that EXPLORER outperforms the baseline agents on Text-World cooking (TW-Cooking) and Text-World Commonsense (TWC) games.

==> sections/3-neuro-symbolic-arch.tex <==
\section{Neuro-Symbolic Architecture for TBGs}
\label{sec:framework}




% need to update the figure
 \begin{figure}[t]
    \centering
    \includegraphics[scale = 0.45]{images/arch_diagram.pdf}
    \caption{Overview of our neuro-symbolic agent's decision-making at any given time step. The Hybrid Neuro-Symbolic architecture mainly consists of 5 modules - (a) \textcolor{Green}{Context Encoder} encodes the observation to dynamic context, (b) \textcolor{SkyBlue}{Action Encoder} encodes the admissible actions, (c) \textcolor{RedViolet!100}{Neural Action Selector} combines (a) and (b) with $\bigoplus$ operator, (d) \textcolor{blue}{Symbolic Action Selector} returns a set of candidate actions, and (e) \textcolor{BurntOrange}{Symbolic Rule Learner} uses ILP and WordNet-based rule generalization to generate symbolic rules.}
    \label{fig:hns_arch}
\end{figure}
 
The main goal of this paper is to demonstrate how a neural and a symbolic agent can work together in an RL environment for TBGs. Neural agents are good at exploration, whereas symbolic agents are good at learning interpretable policies and applying them to select a candidate set of actions. Using this as our motivation, we try to capitalize on the power of both agents to get better results. The key idea is to use the symbolic agent to learn the policies in the form of logic rules and apply them using an ASP solver. When the symbolic agent fails to provide a good action, the neural agent serves as a fallback. In other words, The ``action selector'' in \ex accords priority to the symbolic actions based on the confidence-scores (more details in Appendix-\ref{appx:conf_score}). \ex fallbacks to the neural actions when either of the one following situations happens: (i) no actions or policies for the given state because of early exploration stage or non-rewarded actions, 
 (ii) non-admissible symbolic actions can be generated due to rule generalization. Figure~\ref{fig:hns_arch} illustrates the components of our neuro-symbolic architecture and shows an overview of the agent's decision-making process. 


% In other words, the action selector accords priority to the symbolic agent. 

% The "action selector" in our neuro-symbolic approach tends to select the action of the symbolic agent based on the confidence-scores (more details in Appendix-A). We fallback to the action selected by the neural-agent when one of the following situations happens:
% (i) No actions or policies for the given state because of early exploration stage or non-rewarded actions.
% (ii) Non-admissible symbolic actions can be generated due to rule generalization.


